Scalable Micro-planned Generation of Discourse from Structured Data

We present a framework for generating natural language description from structured data such as tables; the problem comes under the category of data-to-text natural language generation (NLG). Modern data-to-text NLG systems typically employ end-to-end statistical and neural architectures that learn from a limited amount of task-specific labeled data, and therefore, exhibit limited scalability, domain-adaptability, and interpretability. Unlike these systems, ours is a modular, pipeline-based approach, and does not require task-specific parallel data. It rather relies on monolingual corpora and basic off-the-shelf NLP tools. This makes our system more scalable and easily adaptable to newer domains. Our system employs a 3-staged pipeline that: (i) converts entries in the structured data to canonical form, (ii) generates simple sentences for each atomic entry in the canonicalized representation, and (iii) combines the sentences to produce a coherent, fluent and adequate paragraph description through sentence compounding and co-reference replacement modules. Experiments on a benchmark mixed-domain dataset curated for paragraph description from tables reveals the superiority of our system over existing data-to-text approaches. We also demonstrate the robustness of our system in accepting other popular datasets covering diverse data types such as Knowledge Graphs and Key-Value maps.

==> 3_idea.tex <==
\section{Main Idea}
\label{sec:mainidea}
In this section, we discuss techniques and components leading to the generation of paragraph descriptions from tables. Our system embodies a pipeline of three stages, namely, (a) canonicalization, (b) simple language generation, and (c) discourse synthesis and language enrichment. In the first stage the input is converted to a standard canonical representation in the form of tuples. In the second stage each canonical form extracted from the input is converted to simple sentences. In the final stage the simple sentences are merged together to produce complex and more natural sentences. The first stage is essential to handle variable schema and different formats. The second stage gleans morphological, lexical and syntactic constituents from the canonical tuples, and stitches them into simple sentences. \textit{Fig.} \ref{fig:system} gives an overview of our architecture. 

We now describe each of the stages in the following sections. 



==> images/tmp.tex <==
%%%%%%%%%%%%%Triple to Text, Section 4.2 %%%%%%%%%
Here, the context information is provided by the NE tags appearing in the canonical triples. This operation is carried out by our \textsc{Morph} module. This module is again a \texttt{seq2seq} architecture that is trained on a large set of pairs of $<keyword, sentence>$. As of training data, a large number of simple sentences (with one clause) extracted from web-scale text dumps (such as Wikipedia), are processed to automatically generate labeled examples. For instance, stopwords (function words) such as articles and prepositions are dropped from the sentences through a look up. The remaining words are \textit{lemmatized} using a WordNet based lemmatizer, thus producing a key-word list. The key-word lists and sentences act as  labeled data for the system. 

%Most of the times the output generated sentence contains morphological variations of different verbs either from input or added externally, this makes it difficult to have generation across domains due to large number of unknown words. To tackle this challenge we employed a mechanism to generate POS information along with the lemma or base form instead of generating the actual form. The model will generate 'played' from 'play' by generating 'play VBD', similarly, 'was' can be generated as 'is VBZ'. This method combined with the copy mechanism enables the model to learn to produce variations of unknown words by first learning to copy the lemma form and generating variation needed according to the input.} The input to this module, that is, a canonical triple is transformed to a sequence of POS-tagged keywords. POS tagging and stop-word removal is performed on the canonical triple to convert it to this form.
It is necessary to disambiguate the input words to find out the appropriate articles, prepositions and morphological forms of the verbs. To this, we enrich the $<keyword, sentence>$ data and include more information such as POS tags at both input and output side of the training data.  \textit{Figure.} \ref{fig:morph} shows a working example of the \textsc{morph} system.  

For example, the input key-word and POS ``play VERB'' would be translated by the system to ``play VBD'' which will be post-processed to produce  the word ``played'', similarly the auxiliary verb ``was'' can be generated as ``is VBD''. With the current method, a canonical triple like $<$\text{PERSON} \ \text{country played for} \ \text{GPE}$>$ is transformed to the following sequence: \\
\begin{align*}
    \text{\textbf{PERSON} NOUN \textbf{country} NOUN} \\ 
    \text{\textbf{play} VERB \textbf{GPE} NOUN}
\end{align*}
The \texttt{seq2seq} network takes the transformed input and produces an output sequence like
\begin{align*}
    \text{\textbf{PERSON} play VBD for country \textbf{GPE}.}
\end{align*}
The tag `VBD' here is a fine-grained POS tag, which reflects the required inflectional variation of the verb `play'. After normalizing the output sequence taking into account this inflectional variation, the final output of this module is 
\begin{align*}
\text{\textbf{PERSON} \emph{played for country} \textbf{GPE}}. 
\end{align*}

%%%%%%%%%%%%%Experimental Setup%%%%%%%%%%%%%%%
Similar as above, $N-1$ triples are obtained from a \textsc{WikiBio} json and passed to our system to produce a biography description. For the \textsc{WebNLG} dataset, the triples in a group are all consumed together by our system to produce the output. Similarly for \textsc{WikiTablePara} dataset, $M \times (N-1)$ triples lead to the output table description.

    \item \textsc{WikiBioModel} : The \textsc{WebNLG} dataset may have a group of triples producing a text output. Each triple is converted to a JSON as required by the \textsc{WikiBio} format and output is generated from the model. Then these outputs of the group are clubbed and compared with the reference text. Whereas for \textsc{WikiTablePara} dataset, a table consisting $M$ rows and $N$ columns is converted to $M \times (N-1)$ jsons in \textsc{WikiBio} format. Each row represented as \emph{$<$key1:value1, key2:value2, ... , keyN:valueN$>$} is converted to $N-1$ triples $<\text{value}1,\text{key}I,\text{value}I>$ (thus, $N-1$ jsons) assuming the first key is the primary key. The outputs of all $M \times (N-1)$ jsons from the model are concatenated to produce the required table description.
    
We assess the contributions of the individual Triple2Text modules \textsc{multitriple}, \textsc{morph v1} and \textsc{morph v2} followed by analysis of how ranking among them improves the performance (referred as \textsc{ranker} in \emph{Table} \ref{tab:fullablation}). These comparisons are done considering  two scenarios : (1) When sentence compounding is applied followed by coreference replacement (referred as `w' in \emph{Table} \ref{tab:fullablation}), (2) Instead of compounding, simple sentence concatenation is done (referred as `w/o' in the table). Thus, this kind of ablation helps to understand the system across two dimensions, first, the kind of simple sentence generation technique, and second, the kind of language enrichment (whether compounding or concatenation).

%%%%%Related Work%%%
%However, the input they deal with is essentially a set, without any specific order or structure as we are tackling with structured tables. 
\cmmnt{Another relevant work is Neural Knowledge Language Model , which an be trained to generate descriptions for \textit{Freebase} facts. However, this is again a supervised model trained on a parallel dataset.} \cmmnt{unsupervised data-to-text generation \cite{unsupnlg}, }key-word to text generation \cite{reddy2017}, and Set2Seq generation \cite{44871}. \cmmnt{We acknowledge that some of these approaches can be utilized in various modules of our pipeline which would yield a large number of variants of our system. Due to space constraints, we limit our discussion to only the simple models that we propose in the later sections.} 

% To contrast with the above related work we strive to develop a modular, interpretable, data-driven architecture for table to text generation which relies only monolingual unlabelled data which can prove to be robust across domains, languages and structural variations.

%End-to-end DL approaches \cite{N18-1139,N18-2098}
%NLG micro-planning \cite{nlg-micro17}, one-sentence biography from wikidata \cite{E17-1060}. Multiple tables (out of scope) \cite{wiseman2017challenges}. Fixed schema table \cite{N18-2098}. We are extending to variable schema. Story generation \cite{DBLP:journals/corr/JainAMSLS17}. Contrast with Neural Knowledge Language Model \cite{nklm16}. Recent work \cite{D17-1239} had observed that even with recent ideas of copying and reconstruction, there is a significant gap between neural models and template-based systems, highlighting the challenges in data-to-text generation. Unsupervised NLG for structured data \cite{unsupnlg}. Table-to-Text (WIKITABLETEXT) \cite{table2text}. E2E challenge dataset \cite{W17-5525}. Existing datasets limitation \cite{nlg-micro17}  : \emph{they are domain specific, hence, systems learned from them are restricted to generating domain specific, often strongly stereotyped text (eg. weather forecast or soccer game commentator reports).}

%Contrast with OpenIE based generation and Set2Seq \cite{44871} kind of approaches. (also any other keyword-to-text systems \cite{reddy2017}).

%\textcolor{blue}{Lifted from patent about current SOTA}:
%\begin{enumerate}
%     \item They only take a specific kind of input (say table) and can not easily scale to consider input of another kind (say graph).
%     \item Both rule based and data driven systems are NOT scalable across domains where the vocabulary and schema of the structures of the domains vary considerably.
%     \item Rule based systems require huge manual effort to design rules for each domain and Data driven systems require parallel data (containing pairs ) which is elusive.
%     \item Moreover, both rule based and supervised data driven paradigms only generate monotonous outputs (quite robotic) and can not introduce variations at the output side.
% \end{enumerate}

% \textcolor{blue}{Lifted from patent about our system}:
% \begin{enumerate}
%     \item Its ability to scale to any domain as long as large scale domain specific unlabeled texts are available.
%     \item Its ability to deal with inputs of multiple types of structured data with variable structures and from variable domains.
%     \item Its ability to produce variable output descriptions, which is controlled by the user.
% \end{enumerate}

% Comparison of various known struct2text tasks/datasets:

% \begin{table}
% \centering
% \begin{tiny}
% \begin{sc}
% \begin{tabular}{l|c|c|c|c|c|c}
% \toprule
%  Function & Idem & Mono & Tra & Sca & Full & Lip \\
% \midrule 
%  Sparseflex &\checkmark &\cmark&\cmark&\xmark&\cmark&$1/(1-\lambda)$\\
%  Sparse-exp &\xmark &\cmark&\xmark&\xmark&\cmark&$\infty$\\
%  Sparse-sq &\xmark &\xmark&\xmark&\xmark&\cmark&$\infty$\\
% %  Sparse-log &\xmark &\cmark&\xmark&\cmark&\xmark&$\infty$\\
%  Sparsecone &\cmark &\xmark&\checkmark&\checkmark&\xmark&$\infty$\\
%  \textbf{Sparsehourglass} &\cmark &\cmark&\checkmark&\checkmark&\cmark&$(1+1/Kq)$\\
%  Sum Normalization++ &\cmark &\cmark&\xmark&\cmark&\cmark&$\infty$\\
 
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{tiny}
% \caption{Comparisons from datasets. Here \cmark \ denotes `satisfied in general', \xmark \ signifies `not satisfied' and \checkmark says `satisfied for some constant parameter independent of $\bm{z}$'.}
% \label{tab:datasets}
% \end{table}

